$\lambda_0$: Scaling Open-World Egocentric Human Data for Humanoid Loco-Manipulation

Humanoid loco-manipulation requires coordinated whole-body interaction with the physical world, yet collecting robot demonstrations at scale remains costly. Human demonstrations offer a scalable alternative, but existing egocentric human supervision often omits locomotion and posture, while embodiment differences and controller dynamics hinder accurate end-effector execution. We introduce HumanVerse, a 500-hour dataset of open-world human loco-manipulation pairing egocentric video with synchronized body and hand motion. Our human-to-humanoid pipeline aligns camera viewpoints and arm appearance, and refines motion references and controller inputs offline to reduce end-effector errors while preserving whole-body coordination. We validate the pipeline through zero-shot transfer to Unitree G1 on representative whole-body manipulation and long-range loco-manipulation tasks, without target-task robot demonstrations. Building on this pipeline, we develop $\lambda_0$, a humanoid foundation model for whole-body loco-manipulation, with robot-aligned human demonstrations providing supervision for mid-training. Increasing whole-body human data consistently improves downstream task progress. $\lambda_0$ achieves 90.0% success on SIMPLE and 62.5% across real-world loco-manipulation tasks. We expect this study to guide scalable whole-body human data collection toward humanoid foundation models for richer interaction with the physical world. Homepage: https://lambdahumanoid.github.io/

==> figs/generalization_data.tex <==
% Generated by scripts/import-generalization-results.py; do not edit values by hand.
% Feishu revision 4585; 10 trials per task/method/condition.
% Groups: Seen = RH-A; Human-guided = RH-B; Robot-only = R-B.
% Within each group: Pi0.5, GR00T N1.6, Psi0, StarVLA, Lambda0.
\newcommand{\setgeneralizationvalues}[1]{%
  \ifcase#1\relax
    % Toy storage
    \def\genvalues{73,28,38.5,59.5,81,47,13.5,30,30.5,70.5,54.5,9,8.5,26.5,61}
  \or
    % Box transport
    \def\genvalues{67,10,43.5,71,90,59.5,10,37.5,15,61.5,59.5,10,8.5,9,53.5}
  \or
    % Bottle disposal
    \def\genvalues{28,10,34,19,81.5,40.5,5,26.5,13,37,34.5,10,14.5,10,29.5}
  \or
    % Chair placement
    \def\genvalues{65.5,52.5,33,75,81.5,39,30,33,42,54,34,34,30,36,49.5}
  \fi
}

